Dynamics, data and reconstruction

The goal of data-driven learning of dynamical systems is to interpret time series as a continuous observation of an underlying dynamical system. This task is not well-posed for a variety of reasons - such as multiple co-existing sub-systems, topologically inter-weaving of these sub-systems; and more importantly, the non-injectivity of the correspondence between dynamical systems and time series. We show how these ambiguities are circumvented if one considers dynamical systems and measurement maps collectively. Dynamical systems, observed dynamical systems, and time series data - each of these three collections have an extensive network of relations within them, which gives them the mathematical structure of a category. One of the new concepts proposed is a rigorous definition of time series data as a chain of measurement sequences with decreasing information content. This definition subsumes the familiar notions of sequences, time series and even subshifts. Using these notions it is shown that the entire process of converting an observed dynamical systems into a time series object is functorial, and passes through a number of phases each bearing its own categorical structure. This discovery sheds new light on the nature of reconstruction algorithms. Under mild conditions of consistency, reconstruction itself is shown to be functorial operation. This provides a new category theoretic perspective on the nature and limits of reconstruction.

==> Table_TC.tex <==
\begin{tabularx}{\linewidth}{|l|L||l|L|}
	$\calG$ & Interpretation & $\calC$ & Interpretation \\ \hline \hline
	$\real$ & Invertible flow, continuous time & $\Topo$ & Topological dynamics \\ \hline
	$\Rplus$ & Continuous time & $\MeasCat$ & Measurable dynamics \\ \hline
	$\num$ & Discrete time & $\BanachCat$ & Operator family \\ \hline
	$\integer$ & Invertible, Discrete time & $\StochCat$ & Markov process \\ \hline
	$\mathbb{T}^d$ & Torus actions & $\SetCat$ & Set-theoretic dynamics \\ \hline
\end{tabularx}
